Efficient Terrain Stochastic Differential Efficient Terrain Stochastic Differential Equations for Multipurpose Digital Elevation Model Restoration

Digital Elevation Models (DEMs) are indispensable in the fields of remote sensing and photogrammetry, with their refinement and enhancement being critical for a diverse array of applications. Numerous methods have been developed for enhancing DEMs, but most of them concentrate on tackling specific tasks individually. This paper presents a unified generative model for multipurpose DEM restoration, diverging from the conventional approach that typically targets isolated tasks. We modify the mean-reverting stochastic differential equation, to generally refine the DEMs by conditioning on the learned terrain priors. The proposed Efficient Terrain Stochastic Differential Equation (ET-SDE) models DEM degradation through SDE progression and restores it via a simulated reversal process. Leveraging efficient submodules with lightweight channel attention, this adapted SDE boosts DEM quality and streamlines the training process. The experiments show that ET-SDE achieves highly competitive restoration performance on super-resolution, void filling, denoising, and their combinations, compared to the state-of-the-art work. In addition to its restoration capabilities, ET-SDE also demonstrates faster inference speeds and the capacity to generalize across various tasks, particularly for larger patches of DEMs.

==> parts/exp_joint.tex <==
\section{Experiment}
To evaluate the proposed sde4DEM, we first compare it with 3 state-of-the-art (SOTA) deep-learning-based methods and two traditional interpolation-based methods.
\subsection{Implementation Details}
\subsubsection{Dataset and Preprocessing}
\paragraph{Area1: Austria national DTM}
% The data from the Shuttle Radar Topography Mission (SRTM) is primarily led by collaborative efforts between the U.S. National Aeronautics and Space Administration (NASA) and the U.S. National Geospatial-Intelligence Agency (NGA). Covering an expansive area of 119 million km2, the radar images collected are categorized into SRTM1 and SRTM3, corresponding to resolutions of 30m and 90m, respectively (Jarvis, Reuter, Nelson, & Guevara, 2008). Elevation models derived from SRTM data are freely accessible and enjoy widespread file format support. Since its release, SRTM DEM has been extensively utilized in geosciences. This study specifically gathers SRTM DEM data with a resolution of 30m.

Study area-1 was extracted from the Austria National Digital Terrain Model (DTM). This chosen region amalgamates urban and natural landscapes, encompassing plains, hills, mountains, and water systems, rendering it a comprehensive area suitable for testing. The 10m Digital Elevation Model (DEM) of Study Area-2 exhibits an elevation range from 206.588 $m$ to 3337.73m, with an image size of 21046 × 16291, accessible through \url{https://www.data.gv.at/katalog/dataset}.

\paragraph{Area 2: Mount Tai}
Study area-2 is located around Mount Tai, an elevation that ascends abruptly from the extensive plain of central Shandong. This location is inherently adorned with a multitude of scenic sites, characteristic of a tilted fault-block mountain formation.
% 
The area is densely adorned with a profusion of springs, intricately interwoven with a network of rivers and streams. 
%This configuration contributes to the region's relatively abundant water resources.
The elevation of the study area ranges from 3$m$ to 680$m$, which is obtained from 
\url{https://gdemdl.aster.jspacesystems.or.jp/index_en.html}. The Advanced Spaceborne Thermal Emission and Reflection Radiometer (ASTER) is a
14-channel imaging instrument operating on NASA’s Terra satellite. in 16-bit GeoTiff format.



\subsubsection{Metrics}
To comprehensively assess the performance of the super-resolution models, 
\begin{itemize}
    \item MAE (mean absolute error):
    \item RMSE (root mean square error):
    \item PSNR (peak signal to noise ratio):
    \item SSIM (structural similarity index measure): show the visual similarity of the reconstructed data
    \item 
\end{itemize}

\subsection{Comparison with SOTAs on multiscales}
In this section, we validate the effectiveness of the proposed sde4DEM and compare the super-resolution performance of it with 
state-of-the-art methods. 
%
To effectively conduct the comparison, we choose representative models, including both traditional interpolation-based methods and deep-learning-based methods
\begin{itemize}
    \item 
    \item 
    \item
\end{itemize}
The statistical results tested on the TFASR30 dataset are listed in Table~\ref{tab:comp}.

\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\subsection{Ablation studies}
\subsubsection{Ablation study on the feature extraction module}

\subsubsection{Ablation study on loss functions}

% \subsubsection{Possible future direction}



==> parts/exp_oldbk.tex <==

\paragraph{Norway City Dataset and Mount Tai Dataset with Rectangular Voids}
For DEM of size $256 \times 256$, we take the same settings as \cite{diff-dem},
the voids as rectangular patches are randomly exerted on the DEMs with sizes ranging from 64 pixels to 128 pixels.
%
The test collections are selected according to the difficulties, the splits are listed in Table~\ref{tab:masks_patches} with $w_{min}$ to be the minimal patch size, and with $w_{max}$ to be the maximal patch size.

\section{Experiment}
This section evaluates the proposed EGR-SDE for three typical refinements to enhance DEM quality: super-resolution, void filling, and denoising.
EGR-SDE is compared to the state-of-the-art works in the respective fields in Section~
\ref{sec:sr}, ~\ref{sec:voidfill}, % ~\ref{sec:sr_with_voids}, 
and ~\ref{sec:denoise}. 
\subsection{Basic Setup}
\subsubsection{Implementation Details}
The EGR-SDE pipeline for the experiments incorporates 3 TABs in the TPE blocks to enhance the feature extraction with channels set to be 4.
%
The settings of the noise-predicting neural network follows the canonical diffusion pipeline \cite{ir-sde}. The internal channels of the convolutions are set to 64, the encoder contains 14, 1, 1, 1 EABs at each depth, and the decoder holds 1 EAB at each depth.
%
For the super-resolution task, for each batch with a batch size of 4, 500,000 iterations are set for training. The initial learning rate is 4e5, with a cosine scheduler and an AdamW optimizer with $\beta_1=0.9, \beta_2=0.999$.The total diffusion step $T=50$ is set for Pyrenees area with patch size of $96\times 96$, and $T=100$ is set for Pyrenees area with patch size of $256\times 256$.
All the experiments are conducted with PyTorch on one NVIDIA RTX 3090 GPU with 24 GB memory. 
\subsubsection{Metrics and Benchmarks}
To comprehensively evaluate the performance of super-resolution models, we use metrics from both a topological and an image perspective.
\begin{itemize}
    \item MAE (Mean Absolute Error):
    The average of the L1 distance across all grid units between the ground truth and the estimated height map.
    % $MAE_t = \frac{\sum\limits_{i=1}^N\|\hat{h}_i - h_i^{(gt)}\|}{N}$
    \item RMSE (Root Mean Square Error) of altitude: the standard deviation of the residuals between the ground truth and the estimated height map.
    % $RMSE_t = \sqrt{\frac{\sum\limits_{i=1}^N(\hat{h}_i - h_i^{(gt)})^2}{N}}$.
    \item PSNR (Peak Signal to Noise Ratio):
    The ratio between the maximum possible value (power) of a signal and the power of distorting noise that affects the quality of its representation, manifesting the visual fidelity of the restored DEM.
    \item SSIM (Structural Similarity Index Measure): 
    % The visual similarity of the reconstructed data. 
    The perceptual metric that quantifies multiscale DEM quality degradation as an image, with various windows of the DEM patch. 
\end{itemize}

We have chosen the EBCF-CDEM method to represent the deep-learning-based approach for its state-of-the-art performance over various types of methods. No other deep models were used in our study since EBCF-CDEM has reported the best performance. We have also chosen the bicubic interpolation as a representation of the traditional super-resolution method.
%
In the original implementation of EBCF-CDEM, the PSNR is calculated in a cropped sub patch. For fairness, all the metrics are calculated for the whole patch. 
\subsection{DEM super-resolution}
\label{sec:sr}
\subsubsection{Experimental Setup}
\paragraph{Dataset preparation}
% \paragraph{Area 1: Austria National DTM}
% Study area-1 was extracted from the Austria National Digital Terrain Model (DTM). This chosen region amalgamates urban and natural landscapes, encompassing plains, hills, mountains, and water systems, rendering it a comprehensive area suitable for testing. The 10m Digital Elevation Model (DEM) of Study Area-2 exhibits an elevation range from 206.588 $m$ to 3337.73m, with an image size of 21046 × 16291, accessible through \url{https://www.data.gv.at/katalog/dataset}.
To evaluate the robustness and effectiveness of EGR-SDE for super-resolution, 
we adopt DEM from challenging mountainous regions.
%
The study area is located around the Pyrenees mountain.
The DEM data of the Pyrenees has a resolution of 2 meters and is divided into 10 regions, covering a total area of 643 square kilometers in mountainous areas. The large-region DEMs are divided into non-overlapped subtitles, each with a size of 96 × 96. 90\% of the DEM tiles are randomly selected for training, resulting in 15,206 training tiles, while the remaining 10\% are used for testing, totaling 1690 testing tiles. The Pyrenees area is used for the joint restoration task, with the resolution of the low-quality DEM to be 15 meters. 
\paragraph{preprocess}
Among the current state-of-the-art deep learning-based DEM super-resolution works, the algorithms are applied to small DEM patches, such as the newest work EBCF-CDEM \cite{continuous} with the best results are tested with patch size smaller than $100 \times 100$.
Here we test the effectiveness of EGR-SDE with relatively larger DEM patches of $256\times 256$ with two super-resolution of 2 and 4 times of scales. 


\subsubsection{Results of super resolution}
Previous works mostly cropped the DEM into small patches, since some methods gather local information with smaller windows.
While diffusion models (including SDEs), have less dependence on local information. 
Therefore, this section investigates the capability of EGR-SDE on larger DEM patches, with more details and variations within one patch. 
 
The quantitative comparison is shown in %Table~\ref{tab:aster_comp_sotax2} and 
Table~\ref{tab:aster_comp_sotax4}.
% 
Although all the models yield complete results, the result of bicubic interpolation lacks details. Meanwhile, as Fig.~\ref{fig:results_aster} shows, EBCF-CDEM manifests an over-smoothing phenomenon, due to the locally continuous implicit representations. 
%
In comparison, EBCF-CDEM is more suitable for small patches, but EGR-SDE is robust to larger patches.


% \subsection{Comparison of Generalization}
% Apart from evaluating the universality, we also validate the generalization ability of the proposed EGR-SDE over other datasets for testing.
% %





\subsection{DEM void filling}: 
\label{sec:voidfill}
\subsubsection{Experimental Setup}
\paragraph{Dataset preparation}
For DEM void filling, study area 2 is located around Mount Tai, an elevation that ascends abruptly from the extensive plain of central Shandong. This location is adorned with many scenic sites, characteristic of a tilted fault-block mountain formation.%
%
The area is densely adorned with a profusion of springs, intricately interwoven with a network of rivers and streams. 
%This configuration contributes to the region's relatively abundant water resources.
The elevation of the study area ranges from 3$m$ to 680$m$, which is obtained from 
\footnote{\url{https://gdemdl.aster.jspacesystems.or.jp/index_en.html}}, the Advanced Spaceborne Thermal Emission and Reflection Radiometer (ASTER) is a
14-channel imaging instrument operating on NASA’s Terra satellite in 16-bit GeoTiff format.

\paragraph{Preprocess}
For the void filling task,  on the Pyrenees area, $T=100$ and 800,000 iterations are set for training with $\beta_1=0.9, \beta_2=0.5$.

\subsection{DEM denoising}
\label{sec:denoise}

\subsubsection{DEM super-resolution with voids}
\label{sec:sr_with_voids}
\subsubsection{Experimental Setup}
\paragraph{Dataset preparation}
\subsection{Results of  DEM Super-Resolution and Void Filling}
% To validate the effectiveness of the EGR-SDE for low-resolution DEM with voids, this section compares the performance of EGR-SDE and the   
\begin{table}
\centering
\caption{Quantitative Comparison of EGR-SDE with Benchmarks on the Pyrenees Area.}
\begin{tabular}{c|c|cccc}
\toprule
model& mask
 & PSNR&SSIM&MAE&RMSE\\
\midrule
 \multirow{4}{*}{Bicubic} 
  &No Voids&28.57 &0.72 &1.18 &1.71 \\ 
 &M-311&25.36 &0.49 &1.20 & 1.73\\  
 &M-423&17.03 & 0.31&23.61 &682.35\\
  &M-442 &15.54 &0.28 &25.92 &724.93\\ 
  &M-533 &14.39 & 0.30&31.46 &871.44 \\
  \hline
 \multirow{4}{*}{EBCF-CDEM} 
  &No Voids& 39.61&0.95 &0.71 &1.23 \\ 
 &M-311&24.59 & 0.69&0.72 & 1.23\\  
 &M-423&17.37 &0.52 & 24.20&713.28\\
  &M-442 &14.93 &0.39 &24.94 &739.32\\ 
  &M-533 &13.82 & 0.37&30.71 & 841.96\\
  \hline
 \multirow{4}{*}{EGR-SDE}
  &No Voids&36.15 & 0.91&0.59 &1.08 \\ 
 &M-311&32.16 &0.88 & 0.66 & 1.20\\  
 &M-423&29.54 &0.82 &0.73 &1.27\\
  &M-442 &28.75 &0.80 &0.70 &1.25\\ 
  &M-533 &28.03 &0.78 &0.75&1.29 \\
%0.25x-----------------
\bottomrule
\end{tabular}
\label{tab:pyrenees_comp_sota}
\end{table}
\begin{figure*}
\centering
    \includegraphics[width=15cm]{pics/results_aster_comp.png}
    \caption{Qualitative Comparison of EGR-SDE with Benchmarks of 4x Super Resolution on Mountain Tai Area. %For larger input size, EBCF-CDEM exhibits over-smoothness for details, while EGR-SDE preserves the granularity.
    }
    \label{fig:results_aster}
\end{figure*}


\begin{table}
\centering
\caption{Quantitative Comparison of EGR-SDE with On Larger Patches of the Mountain Tai of 2x Super-Resolution.}
\begin{tabular}{c|ccc}
\toprule
model& Bicubic & EBCF-CDEM &EGR-SDE\\
\midrule
PSNR &22.39&21.44 &\textbf{26.51}\\
SSIM &0.65 & 0.67&\textbf{0.75} \\
MAE & 4.31&3.28&\textbf{0.93}\\
RMSE &6.22&5.41&\textbf{1.12} \\
\bottomrule
\end{tabular}
\label{tab:aster_comp_sotax4}
\end{table}

\subsubsection{Comparison with Benchmarks}

Table~\ref{tab:pyrenees_comp_sota} reports the comparison between the benchmarks with different levels of voids. The comparison is conducted on the masked Pyrenees area, the goal is to enhance the quality of DEM patches of 15m-resolution to 2m-resolution with randomly masked null values.
When there are no voids exerted on the DEM patch, the problem degenerates to common DEM super-resolution task.
% Since the patch size is quite small, 
From Table~\ref{tab:pyrenees_comp_sota},  EBCF-CDEM and EGR-SDE manifest similar performance for patches without voids.
However, when the voids become more or larger, bicubic interpolation and EBCF-CDEM become more and more ineffective.
\begin{figure}[H]
    \centering
    \includegraphics[width=8.5cm]{pics/sr_with_voids_comp.png}
    \caption{Comparison between different models for restoring digital elevation models (DEMs) using the Pyrenees dataset. The study found that for super-resolution of DEMs without voids, EGR-SDE performs similarly to EBCF-CDEM. When voids are present, and their sizes are smaller than the local coordinates of EBCF-CDEM, they have little negative impact on all the models. However, as the voids increase in size and amount, both interpolation and EBCF-CDEM become less effective.}
    \label{fig:results_pyr_comp_with_voids}
\end{figure}

Visually, from Fig.~\ref{fig:results_pyr_comp_with_voids}, the reason for the performance decrease of all the methods is obvious. Bicubic interpolation and EBCF-CDEM fail to fill the relatively larger voids. 
When the void is small, \eg a hole covering 1 to 2 units within the coordinate, the null values play little negative effects on the whole performance.
For both the bicubic interpolation and EBCF-CDEM, the prediction of the unknown values relies on gathering neighboring information by some means.
This way is effective when the local information can be accessed in a regular pattern. For instance, interpolation methods rely on the neighboring regular grid without nullity, and EBCF-CDEM requires pre-defined local window sizes as hyperparameters to form local retrievable coordinates.
However, when the void size becomes uncontrollable, it is hard to decide the local coordinate, especially when the efficiency is taken into account.
While the diffusion model has no specific requirements for such hyperparameters, and the performance becomes imperfect when adding larger voids, it is still robust and competent compared to the benchmarks.


\subsection{Ablation Study}
\subsubsection{Study of the Gradient Loss}
To investigate the influence of adopting the submodules of the EGR-SDE, this subsection conducts extensive experiments  
\subsection{Controlled Experiments}

\subsubsection{Study of the Total Step $T$ for Larger Patches}
This subsection investigates the effect of the total step $T$ for different patches.

\subsubsection{Comparison on Hyperparameters and Convergence}
For different levels of voids, the EGR-SDE itself should also be adjusted.
Table~\ref{tab:pyrenees_comp_sota} not only manifests the robustness of EGR-SDE against larger voids but also shows the performance degradation for EGR-SDE itself.
Fig.~\ref{fig:sr_with_voids} shows the validation results at different iterations with different levels of voids applied.
It reveals the fact when more and larger voids are added to the DEM, it requires more iterations for EGR-SDE to converge in the training phase. Besides, in the experiments, $T = 60$ is enough for DEM without or with small voids, while $T=100$ suits larger voids.
For the results reported in Table~\ref{tab:pyrenees_comp_sota}, 
% the settings of $T$ is recorded in Table~\ref
$T=60$ for DEM with no voids, with M-311 and M-442, and $T=100$ for DEM with M-423 and M-533.



\begin{figure}[H]
    \centering
    \includegraphics[width=17cm]{pics/sr_with_voids.png}
    \caption{Visualization of the restoration process with different levels of voids to be filled. In (a), the training loss converges fast. In (b), for DEM with M-311, as optimization proceeds, the small voids are firstly tackled, and then the content of the DEM gradually tends to correctness. In (c), it takes much more iterations to handle the voids.}
    \label{fig:sr_with_voids}
\end{figure}








==> parts/intro_old.tex <==
\section{Introduction}
In recent years, the demand for high-resolution geospatial data has intensified across various scientific disciplines, driven by burgeoning applications in environmental monitoring, urban planning, and natural resource management (\cite{dem_assess_review,dem_accuracy_review}). 
Digital Elevation Models (DEMs) serve as fundamental components in geospatial analysis, providing critical information about the Earth's topography, water resource management, and hydrological modeling (\cite{hydrology,dem_landslides}). 
Recent advancements in measurement technologies, exemplified by synthetic aperture radar, have empowered researchers to generate expansive Digital Elevation Models (DEMs) covering large geographical areas. Nevertheless, the constrained precision of these measurement instruments significantly affects the accessibility of high-resolution DEMs, which are indispensable for terrain analysis. Besides, Terrain features are inherently multiscale (\cite{dem_terrain,sota_dem_review}), and the scale conversion between DEMs emerges as a crucial concern in the field of geomorphometry. 

% the related work
% interpolation
Early attempts focused on interpolation techniques to estimate intermediate elevations between existing data points, including inverse-distance-weighted (\cite{IDW}), natural nearest neighbor interpolation (\cite{naturalneighbor}), spline interpolation (\cite{comp_inter17}), \etc. 
Another branch of methods utilizes geostatistical information, such as Kriging (\cite{kriging}) and its variants.
However, these methods could not capture fine-scale details and often resulted in artifacts (\cite{comp_inter17,comp-inter19}).


% other dl
As deep learning methods for single-image super-resolution (SISR) have advanced, more studies address Digital Elevation Model (DEM) tasks by adopting models analogous to those used in SISR.
%
Several studies have arisen to apply high-performing image Super-Resolution (SR) models to DEM SR.
CNN was first employed in DEM Super-Resolution (DEM SR) in D-SRCNN (\cite{cnn1st_dem}), incorporating the architecture of SRCNN and facilitating the transition from image SR to DEM SR.
Xu et al. (\cite{nonlocal}) introduced an initial nonlocal algorithm incorporating high-frequency information from learning examples, demonstrating superior outcomes compared to interpolation-based methods.  Another contribution by Xu et al. (\cite(gradient)) presented a deep gradient prior network for DEM SR, leveraging the EDSR network architecture and integrating gradient loss in the training process. Later, multiscale supervision (\cite{multiscale}), recursive feature extractor (\cite{rspcn}), \etc have further enhanced the network representation capability. To better adapt to terrain properties, (\cite{ridgeline}) further utilizes fused topological information as supervision, and (\cite{terrainfeatureaware}) adaptively optimizes the feature extracting module via deformable convolution.
With the development of generative SISR models, generative adversarial networks (GANs) are progressively introduced to the DEM super-resolution domain. D-SRGAN (\cite{d-srgan}), 
% merely learning the mappings between the low-resolution grid and the high-resolution grid turns out to be 

% generagive 

However, the GAN-based model is vulnerable to mode corruption and unstable optimization (\cite{sisr_review, gan_review}). Additionally, the GAN-based models handle degradation removal and detail refinement simultaneously for the entire image grid. In contrast, diffusion models (DMs) have demonstrated notable success in image restoration (IR), exhibiting finer details and a more straightforward training process (\cite{diffusion_review}). This novel branch of generative models, diffusion models, has recently yielded significant advancements in visual generation and restoration tasks.


% applying diffusion models
This paper fully leverages the continuous diffusion probabilistic modeling to DEM super-resolution task.
Generally, SDE methods used in IR tasks entail gradually diffusing images towards a pure noise distribution using an SDE, and then generating samples by learning and simulating the corresponding reverse-time SDE.
 


